GPT-4 as a Homework Tutor can Improve Student Engagement and Learning Outcomes

This work contributes to the scarce empirical literature on LLM-based interactive homework in real-world educational settings and offers a practical, scalable solution for improving homework in schools. Homework is an important part of education in schools across the world, but in order to maximize benefit, it needs to be accompanied with feedback and followup questions. We developed a prompting strategy that enables GPT-4 to conduct interactive homework sessions for high-school students learning English as a second language. Our strategy requires minimal efforts in content preparation, one of the key challenges of alternatives like home tutors or ITSs. We carried out a Randomized Controlled Trial (RCT) in four high-school classes, replacing traditional homework with GPT-4 homework sessions for the treatment group. We observed significant improvements in learning outcomes, specifically a greater gain in grammar, and student engagement. In addition, students reported high levels of satisfaction with the system and wanted to continue using it after the end of the RCT.

==> tables/data_labels.tex <==

\begin{longtable}{p{0.35\textwidth} p{0.6\textwidth}}
\caption{Data Labels.} \\
\toprule
\textbf{Label} & \textbf{Full Question - English Translation} \\
\midrule
\endfirsthead

\multicolumn{2}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{Label} & \textbf{Full Question - English Translation} \\
\midrule
\endhead

\midrule
\multicolumn{2}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

Ability to Finish Homework & I have the personal abilities to properly complete the English homework every time (this question refers to your personal abilities: your knowledge, being gifted for languages, …). \\ \midrule
Ability to Keep Up & I have the personal abilities to keep up with the English program (this question refers to your personal abilities: your knowledge, being gifted for languages, …). \\ \midrule
Can't Learn English & No matter how hard I try, I can't learn English. \\ \midrule
Confidence in Ability & I think I have the ability to reach a good level of English (approximately a C1) in the coming years (this question refers to your personal abilities: aptitude, being gifted for languages, …). \\ \midrule
Confident in English & In English, no matter how difficult a topic is, I'm sure I can understand it. \\ \midrule
Confident in Tests & I am confident that I can do well in English quizzes, oral exams, and/or tests. \\ \midrule
Doubt in Learning Difficult Topics & I'm not sure I can learn the most difficult topics in the English program. \\ \midrule
Goal for English Level C1 & I want to reach a good level of English in the coming years (approximately a C1). \\ \midrule
Good at Languages & I am gifted for languages. \\ \midrule
Homework Boring & English homework is boring. \\ \midrule
Homework Future Knowledge & English homework is useful for gaining knowledge that will serve me in the future. \\ \midrule
Homework Improves English & English homework is useful for improving my English level. \\ \midrule
Lessons Future Knowledge & English lessons provide me with useful knowledge for my future. \\ \midrule
Lessons Improved English & English lessons are useful for improving my English level. \\ \midrule
Need Support for Homework & I would need more support and resources to be able to do English homework (this question refers to external resources: materials, explanations, feedback on your work, …). \\ \midrule
Need Support to Keep Up & I would need more support and resources to be able to keep up with the English program (this question refers to external resources: materials, explanations, feedback on your work, …). \\ \midrule
Overall Satisfaction & Overall, I am satisfied with what I learn in English at school. \\ \midrule
Satisfied with Homework & I am satisfied with what I learn by doing English homework. \\ \midrule
Skip Hard Exercises & When an exercise is too difficult, I skip it or only do the easier parts. \\ \midrule
Skip Hard Topics & When a topic is too difficult, I skip it and do not try to learn it. \\ \midrule
Struggled with English & I struggle to keep up with the English program. \\ \midrule
Uninterested in Content & The contents of the English program do not interest me. \\
\label{tab:data_labels}
\end{longtable}


==> tables/exercise.tex <==

\begin{table}[]
\begin{tabular}{|c|c|cc|cc|c|}
\hline
\rowcolor[HTML]{000000} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }                                                                      & \cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }                                                                    & \multicolumn{2}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \EC}}                                                                                     & \multicolumn{2}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \EI}}                                                                                     & {\color[HTML]{FFFFFF} }                  \\ \cline{3-7} 
\rowcolor[HTML]{000000} 
\multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}From\\ Week\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}To\\ Week\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} Cohen's d}} & \multicolumn{1}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} P-value}} & \multicolumn{1}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} Cohen's d}} & \multicolumn{1}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} P-value}} & {\color[HTML]{FFFFFF} Number of Samples} \\ \hline
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 1}                                                                                             & {\color[HTML]{212121} 2}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.422}}    & {\color[HTML]{212121} 0.143}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.259}}    & {\color[HTML]{212121} 0.254}                                                & {\color[HTML]{212121} 23}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 1}                                                                                             & {\color[HTML]{212121} 3}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.094}}     & {\color[HTML]{212121} 0.632}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.088}}     & {\color[HTML]{212121} 0.694}                                                & {\color[HTML]{212121} 20}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 1}                                                                                             & {\color[HTML]{212121} 4}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.109}}     & {\color[HTML]{212121} 0.768}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.114}}    & {\color[HTML]{212121} 0.695}                                                & {\color[HTML]{212121} 17}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 1}                                                                                             & {\color[HTML]{212121} 5}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.789}}     & {\color[HTML]{212121} 0.048}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.335}}     & {\color[HTML]{212121} 0.340}                                                & {\color[HTML]{212121} 14}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 1}                                                                                             & {\color[HTML]{212121} 6}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.103}}     & {\color[HTML]{212121} 0.759}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.269}}    & {\color[HTML]{212121} 0.286}                                                & {\color[HTML]{212121} 18}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 2}                                                                                             & {\color[HTML]{212121} 3}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.624}}     & {\color[HTML]{212121} 0.049}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.546}}     & {\color[HTML]{212121} 0.068}                                                & {\color[HTML]{212121} 18}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 2}                                                                                             & {\color[HTML]{212121} 4}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.357}}     & {\color[HTML]{212121} 0.225}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.326}}     & {\color[HTML]{212121} 0.279}                                                & {\color[HTML]{212121} 16}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 2}                                                                                             & {\color[HTML]{212121} 5}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.339}}     & {\color[HTML]{212121} 0.420}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.357}}     & {\color[HTML]{212121} 0.231}                                                & {\color[HTML]{212121} 13}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 2}                                                                                             & {\color[HTML]{212121} 6}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.288}}     & {\color[HTML]{212121} 0.213}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.086}}     & {\color[HTML]{212121} 0.541}                                                & {\color[HTML]{212121} 17}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 3}                                                                                             & {\color[HTML]{212121} 4}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.092}}    & {\color[HTML]{212121} 0.705}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.157}}    & {\color[HTML]{212121} 0.612}                                                & {\color[HTML]{212121} 17}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 3}                                                                                             & {\color[HTML]{212121} 5}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.053}}     & {\color[HTML]{212121} 0.832}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.497}}    & {\color[HTML]{212121} 0.121}                                                & {\color[HTML]{212121} 11}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 3}                                                                                             & {\color[HTML]{212121} 6}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.366}}    & {\color[HTML]{212121} 0.191}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.721}}    & {\color[HTML]{212121} 0.046}                                                & {\color[HTML]{212121} 13}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 4}                                                                                             & {\color[HTML]{212121} 5}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} 0.000}}     & {\color[HTML]{212121} 1.000}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.343}}    & {\color[HTML]{212121} 0.275}                                                & {\color[HTML]{212121} 7}                 \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 4}                                                                                             & {\color[HTML]{212121} 6}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.110}}    & {\color[HTML]{212121} 0.643}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.210}}    & {\color[HTML]{212121} 0.486}                                                & {\color[HTML]{212121} 12}                \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{212121} 5}                                                                                             & {\color[HTML]{212121} 6}                                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.365}}    & {\color[HTML]{212121} 0.285}                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{212121} -0.280}}    & {\color[HTML]{212121} 0.351}                                                & {\color[HTML]{212121} 12}                \\ \hline
\end{tabular}
\caption{Paired t-tests for self reported \EC and \EI across weeks}
\label{tab:exc}
\end{table}

==> tables/exercise_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{scriptsize}
\begin{longtable}{|p{=0.03\linewidth}|p{=0.03\linewidth}|p{=0.03\linewidth}|p{=0.35\linewidth}|p{=0.1\linewidth}|p{=0.35\linewidth}|}
\hline
Cls. & Wk. & Ex. No & Purpose of Exercise                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & Excercise Type                    & Description    \\ \hline\hline
\endhead
3d   & 1    & 1      & Students should learn proper grammar   constructs such as Conditionals Students should be trained to identify and   correct common errors in grammar, syntax, and vocabulary Students should   become more aware of their own weaknesses and their areas for improvement                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Sentence Correction               & Students are asked to correct the mistakes   they will find in each sentence. There is just one mistake in each sentence.                                                                                                                                                                                                                                                                                                                    \\\hline
3d   & 1    & 1      & Students should learn proper grammar   constructs such as Conditionals Students should be trained to identify and   correct common errors in grammar, syntax, and vocabulary Students should   become more aware of their own weaknesses and their areas for improvement                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Sentence Correction               & Students are asked to correct the mistakes   they will find in each sentence. There is just one mistake in each sentence.                                                                                                                                                                                                                                                                                                                    \\ \hline
3c   & 1    & 1      & Students should learn proper grammar constructs such as Conditionals   Students should be trained to identify and correct common errors in grammar,   syntax, and vocabulary Students should become more aware of their own   weaknesses and their areas for improvement                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Sentence Correction               & Students are asked to correct the mistakes they will find in each   sentence. There is just one mistake in each sentence.                                                                                                                                                                                                                                                                                                                    \\ \hline
3c   & 1    & 2      & Students should learn proper grammar constructs such as Conditionals   Students should reinforce sentence structure and word order Students should   practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense to use in the   zero, first, second and third conditional. There may be more than one word.                                                                                                                                                                                                            \\ \hline
3c   & 1    & 3      & Students should learn proper grammar constructs such as Conditionals   Students should learn how to express the same idea in different ways Students   should deepen their understanding of the relationships among different parts   of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Sentence transformation           & Students should complete the second sentence so that it has a similar   meaning to the first sentence. They must use the word given in capital   letters at the end of the line and they cannot change it. They have no   restrictions about the number of words they have to use.                                                                                                                                                           \\ \hline
3c   & 2    & 1      & Students should learn and practice specific expressions such as If only/I   wish and grammar constructs such as mixed conditionals  Students learn to select the correct verbal   tense for the given sentence based on the context in sentences using I wish /   if only and similar mixed conditionals constructs.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & Either/or questions               & Students are given a list of sentences using I wish / if only as well   mixed conditionals. For each sentence, they have to choose the verb in the   correct form among two options that are given to them.                                                                                                                                                                                                                                  \\ \hline
3c   & 2    & 2      & Students should learn proper grammar constructs such as Mixed   Conditionals, If only/I wish Students should reinforce sentence structure and   word order Students should practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & Mixed conditional/ If only/I wish & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense they have to use   in sentences with mixed conditional and with expressions If only/I wish.   There may be more than one word.                                                                                                                                                                         \\ \hline
3c   & 3    & 1      & Writing an argumentative essay on a contemporary social issue. Students   learn to express and argue in favor of a point and discuss counter arguments.   Students should learn proper sentence constructs such as on one hand, on the   other hand, …                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Essay                             & Students are asked to write a short essay about a contemporary social   issue, such as AI, social media, climate change… The essay should be approx.   200-220-word long.                                                                                                                                                                                                                                                                    \\ \hline
3c   & 4    & 1      & To transform sentences from active to passive form keeping the same   tense. Students should learn proper grammar constructs such as Passive form.   Students should learn how to express the same idea in different ways.   Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & Sentence Transformation           & Students are given a sentence in the active form, and need to rewrite in   passive form keeping the same meaning. They have no restrictions about the   number of words they have to use. They must use the same tense when   transforming the sentence from active to passive. Sometimes there is more   than one way to do it.                                                                                                             \\ \hline
3c   & 4    & 2      & To complete the sentences with the correct tense of the verb in brackets.   Students should learn proper grammar constructs such as Passive form Students   should reinforce sentence structure and word order Students should practice   conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets, correctly using active and passive forms. There may   be more than one word.                                                                                                                                                                                                                                                            \\ \hline
3c   & 4    & 3      & Selecting the correct tense: passive or active form Students should learn   and practice specific construct such as passive form Students learn to select   the correct verbal tense and form (active or passive) for the given sentence   based on the context                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & Either/Or Questions               & Students are given a list of sentences. For each sentence, they have to   choose both the form (active or passive) and the verb in the correct form   between two options that are given to them.                                                                                                                                                                                                                                            \\ \hline
3c   & 5    & 1      & Students should learn proper grammar constructs such as have/get   something done Students should reinforce sentence structure and word order   Students should practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense they have to use   and how to use the construct “have/get something done”. There may be more   than one word.                                                                                                                                                                                          \\ \hline
3c   & 5    & 2      & Students should learn proper grammar constructs such as Passive form with   double object Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & Sentence Transformation           & Students should transform the given sentences preserving the original   meaning. First they should transform it in simple passive form (with single   object), and then they should transform it in passive form with double   object. They have no restrictions about the number of words they have to use.   They must use the same tense when transforming the sentence from active to   passive. Sometimes there are more ways to do it. \\ \hline
3c   & 6    & 1      & Students should learn proper grammar constructs such as reported speech   statements Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Sentence Transformation 1         & Students should transform the first sentence which presents a direct   speech statement  into a second   sentence which will present a reported speech one. Students must be careful   when choosing the correct tense according to the introductory verb which is   already given (e.g., Lara said)                                                                                                                                         \\ \hline
3c   & 6    & 2      & Students should learn proper grammar constructs such as reported speech   questions Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & Sentence Transformation 2         & Students should transform the first sentence which presents a direct   speech question into a second sentence which will present a reported speech   one. Students must be careful when choosing the correct tense according to   the introductory verb which is already given (e.g., Lara asked)                                                                                                                                            \\ \hline
3c   & 6    & 3      & Students should learn proper grammar constructs such as reported speech   with different reporting verbs Students should be trained to identify and   correct common errors in grammar, syntax, and vocabulary Students should   become more aware of their own weaknesses and their areas for improvement                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Sentence Correction               & Students are asked to correct the mistakes they will find in each   sentence. There is just one mistake in each sentence.                                                                                                                                                                                                                                                                                                                    \\ \hline
3d   & 1    & 2      & Students should learn proper grammar constructs such as Conditionals   Students should reinforce sentence structure and word order Students should   practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense to use in the   zero, first, second and third conditional. There may be more than one word.                                                                                                                                                                                                            \\ \hline
3d   & 1    & 3      & Students should learn proper grammar constructs such as Conditionals   Students should learn how to express the same idea in different ways Students   should deepen their understanding of the relationships among different parts   of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & Sentence transformation           & Students should complete the second sentence so that it has a similar   meaning to the first sentence. They must use the word given in capital   letters at the end of the line and they cannot change it. They have no   restrictions about the number of words they have to use.                                                                                                                                                           \\ \hline
3d   & 2    & 1      & Students should learn and practice specific expressions such as If only/I   wish and grammar constructs such as mixed conditionals  Students learn to select the correct verbal   tense for the given sentence based on the context in sentences using I wish /   if only and similar mixed conditionals constructs.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & Either/or questions               & Students are given a list of sentences using I wish / if only as well   mixed conditionals. For each sentence, they have to choose the verb in the   correct form among two options that are given to them.                                                                                                                                                                                                                                  \\ \hline
3d   & 2    & 2      & Students should learn proper grammar constructs such as Mixed   Conditionals, If only/I wish Students should reinforce sentence structure and   word order Students should practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & Mixed conditional/ If only/I wish & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense they have to use   in sentences with mixed conditional and with expressions If only/I wish.   There may be more than one word.                                                                                                                                                                         \\ \hline
3d   & 3    & 1      & Writing an argumentative essay on a contemporary social issue. Students   learn to express and argue in favor of a point and discuss counter arguments.   Students should learn proper sentence constructs such as on one hand, on the   other hand, …                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Essay                             & Students are asked to write a short essay about a contemporary social   issue, such as AI, social media, climate change… The essay should be approx.   200-220-word long.                                                                                                                                                                                                                                                                    \\ \hline
3d   & 4    & 1      & To transform sentences from active to passive form keeping the same   tense. Students should learn proper grammar constructs such as Passive form.   Students should learn how to express the same idea in different ways.   Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & Sentence Transformation           & Students are given a sentence in the active form, and need to rewrite in   passive form keeping the same meaning. They have no restrictions about the   number of words they have to use. They must use the same tense when   transforming the sentence from active to passive. Sometimes there is more   than one way to do it.                                                                                                             \\ \hline
3d   & 4    & 2      & To complete the sentences with the correct tense of the verb in brackets.   Students should learn proper grammar constructs such as Passive form Students   should reinforce sentence structure and word order Students should practice   conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets, correctly using active and passive forms. There may   be more than one word.                                                                                                                                                                                                                                                            \\ \hline
3d   & 4    & 3      & Selecting the correct tense: passive or active form Students should learn   and practice specific construct such as passive form Students learn to select   the correct verbal tense and form (active or passive) for the given sentence   based on the context                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & Either/Or Questions               & Students are given a list of sentences. For each sentence, they have to   choose both the form (active or passive) and the verb in the correct form   between two options that are given to them.                                                                                                                                                                                                                                            \\ \hline
3d   & 5    & 1      & Students should learn proper grammar constructs such as have/get   something done Students should reinforce sentence structure and word order   Students should practice conjugating verbs                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Sentence Completion               & Students are asked to complete the sentences with the most suitable form   of the verbs in brackets. They must understand which tense they have to use   and how to use the construct “have/get something done”. There may be more   than one word.                                                                                                                                                                                          \\ \hline
3d   & 5    & 2      & Students should learn proper grammar constructs such as Passive form with   double object Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & Sentence Transformation           & Students should transform the given sentences preserving the original   meaning. First they should transform it in simple passive form (with single   object), and then they should transform it in passive form with double   object. They have no restrictions about the number of words they have to use.   They must use the same tense when transforming the sentence from active to   passive. Sometimes there are more ways to do it. \\ \hline
3d   & 6    & 1      & Students should learn proper grammar constructs such as reported speech   statements Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Sentence Transformation 1         & Students should transform the first sentence which presents a direct   speech statement  into a second   sentence which will present a reported speech one. Students must be careful   when choosing the correct tense according to the introductory verb which is   already given (e.g., Lara said)                                                                                                                                         \\ \hline
3d   & 6    & 2      & Students should learn proper grammar constructs such as reported speech   questions Students should learn how to express the same idea in different   ways Students should deepen their understanding of the relationships among   different parts of speech and sentence structures.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & Sentence Transformation 2         & Students should transform the first sentence which presents a direct   speech question into a second sentence which will present a reported speech   one. Students must be careful when choosing the correct tense according to   the introductory verb which is already given (e.g., Lara asked)                                                                                                                                            \\ \hline
3d   & 6    & 3      & Students should learn proper grammar constructs such as reported speech   with different reporting verbs Students should be trained to identify and   correct common errors in grammar, syntax, and vocabulary Students should   become more aware of their own weaknesses and their areas for improvement                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Sentence Correction               & Students are asked to correct the mistakes they will find in each   sentence. There is just one mistake in each sentence.                                                                                                                                                                                                                                                                                                                    \\ \hline
5c   & 1    & 1      & Students should be encouraged to develop critical thinking Students   should be able to analyze, evaluate and synthetase information Students   should draw on their knowledge and apply it to new situations                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & Questions on the war              & Students are asked to answer two open questions about WWI and British   people’s reaction and reception ( 8-10 lines ).                                                                                                                                                                                                                                                                                                                      \\ \hline
5c   & 2    & 1      & Students should be able to understand the themes, meaning and literary   devices used in the two poems (The soldier by R. Brooke and Dulce et Decorum   est by W. Owen) Students should be able to interpret the poem’s message,   symbolism and imagery Students should improve their writing skills by   conveying their ideas clearly and coherently in a written commentary format                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Poem Commentary                   & Students are asked to write a commentary, analyzing and comparing the two   poems: The soldier by R. Brooke and Dulce et Decorum est by W. Owen. they   must define the main themes of the two poems and the different and   contrasting ways in which war is described. Students must understand the main   themes, the key words and their meaning; they must look for rhetorical   devices and try to interpret the message of the poems. \\ \hline
5c   & 3    & 1      & Students should practice their knowledge of key events of the XXth   century they discussed in class. Specifically, they know the key following   facts about 3 main topics: 1- 1967 as Annus Mirabilis 1967 was an annus   mirabilis as regards sexual mores: Abortion Act National Health Service   (Family Planning) Act (local authorities provide contraceptives) Sexual   Offences Act(It decriminalised homosexual acts in private between two men   over 21) Divorce Act (1969) Matrimonial Property Act (1970) (the wife‚Äôs work   was regarded as an equal contribution towards creating the Family home) 2-   WW2 Participants: World War II (1939-45), major belligerents - Axis (Germany,   Italy, Japan) vs Allies (France, Britain, USA, Soviet Union, China). Initial   Events: 1938, Germany annexes Czechoslovakia; 1939, invades Poland,   triggering WWII. Turning Points: Failure of Germany to control air, 1940.   Invasion of USSR by Germany, 1941; severe losses due to Russian winter and   resistance. USA enters war, 1941 post-Pearl Harbor attack. Conclusion: D-Day,   1944: Allied forces land in Normandy. Germany surrenders, 1945,   post-Hitler‚Äôs suicide. USA drops atomic bombs on Hiroshima, Nagasaki, 1945,   leading to Japan's surrender. 3- Margaret Thatcher 4th May 1979: Margaret   Thatcher (right wing of theConservative Party) became Prime Minister. She   tried to solve the UK‚Äôs economic decline and to reduce the role of the   state in the economy.                                             & Questions on the 20th century     & Students are asked to answer one open question for each of the following   topics: 1. 1967, annus mirabilis 2. Key points of WW2 3. Margaret Thatcher                                                                                                                                                                                                                                                                                        \\ \hline
5c   & 4    & 1      & Students should practice their knowledge of key events of the 20s in the   US they discussed in class. Specifically, they know the key following facts   about 4 main topics: 1- Economical changes Reasons for prosperity in the 20s:   Impact of the car industry Impact of Ford’s assembly line Development of car,   electrical and radio and motion picture industry,  Consequences: economical boom, Mass   consumption  2- political changes  US between 1920-1930 was led by Republican   presidents that try to return to normality after WWI Under president Hoover   there was the Wall Street Crash (Black Tuesday) in 1929 Beginning of the   Great Depression  3- social Changes   1919: 18th amendment and beginning of prohibition: bootlegging 1920: 19th   amendment: women can vote 1933 21st amendment made alcohol legal again   Speakeasies and flappers Nativism and racism     4-  F. S. Fitzgerald: The Great   Gatsby Main points of his life: Zelda, excess, the Lost Generation The Great   Gatsby: main characters  The Great   Gatsby: setting (Valley of Ashes, East/West Eggs, New York The Great Gatsby:   main themes (old money v new money,, self-made man, cars, the American dream)   The Great Gatsby: symbols (green light, Valley of Ashes, East/West Eggs)                                                                                                                                                                                                                                                           & Questions on the Roaring 20s      & Students are asked to answer one open question for each of the following   topics: 1. Reasons for prosperity in the US 20s 2. Great Depression 3.   Prohibition 4. The Great Gatsby                                                                                                                                                                                                                                                          \\ \hline
5c   & 5    & 1      & Students should practice their knowledge of key events after WWII  in the US they discussed in class.   Specifically, they know the key following facts about 4 main topics: Cold   War:  Dates countries involved Reasons   The Swinging Sixties: Some key dates: 1961: Kennedy’s election and the   Soviet’s first manned spaceflight 1962: Nuclear showdown with Cuba 1963:   Kennedy’s assassination 1964: Civil Rights Act 1969: USA moon landing The   cultural revolution: drugs, discos,    progressiveness in education, pop music and poetry, one-parent   families,  the contraceptive pill,   abortion homosexuality legalised. The decay of the 70s: 1959-75 Vietnam War   and protests 1972-1974: The Watergate scandal 1970s: Carter’s administration   was marked by stagflation (stagnation+inflation = slow economic growth and   rising prices) ‘Me’ decade    Individualism, selfishness, punk culture, political struggle,   radicalism (no pacifism), racism, nihilism                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & Open Questions                    & Students are asked to answer one open question for each of the following   topics: 1. Main reasons and beginning of cold War 2. Most important dates of   the 60s in the US with main events 3. Essential aspects of the US cultural   revolution 4. Crisis of the 70s                                                                                                                                                                       \\ \hline
5c   & 6    & 1      & Students should practice their knowledge of the most important activists   for Human Rights they discussed in class. Specifically, they know the key   following facts about the following main topics:  Gandhi’s life: In May 1883, he was married   to 14-year old girl (arranged marriage) In 1888 Gandhi travelled to London,   to study law at University College London and to train as a lawyer. His   attempts at establishing a law practice in Mumbai failed. In 1893 he went to   South Africa and faced discrimination (concept of apartheid) In 1920 he   became leader of the Indian National Congress In 1934 he resigned not only as   the leader but also as a member of theCongress Party. Gandhi was assassinated   in 1948 2. Gandhi’s main achievements and influence The non violent   resistance: satyagraha. His methods included writing speeches and letters   leading marches organizing protests and demonstrations boycotting British   goods and institutions leading prayer meetings 1930: the Salt March: a   satyagraha against the British-imposed tax on salt, which affected the   poorest section of the community. It resulted in the imprisonment of more   than 60,000 people. Quit India: This was Gandhi's and the Congress Party's   most definitive revolt aimed at securing the British exit from India.   formation of the two new dominions of India and Pakistan in mid-August 1947.   His Legacy of nonviolence and civil rights influenced many leaders worldwide   such as Nelson Mandela and M.L. King Jr. & Open Questions                    & Students are asked to answer 5 open questions on Gandhi’s life and   achievements.                                                                                                                                                                                                                                                                                                                                                           \\ \hline
5d   & 1    & 1      & Students should be able to understand the themes, meaning and literary   devices used in the two poems (The soldier by R. Brooke and Dulce et Decorum   est by W. Owen) Students should be able to interpret the poem’s message,   symbolism and imagery Students should improve their writing skills by   conveying their ideas clearly and coherently in a written commentary format                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Poem Commentary                   & Students are asked to write a commentary, analyzing and comparing the two   poems: The soldier by R. Brooke and Dulce et Decorum est by W. Owen. they   must define the main themes of the two poems and the different and   contrasting ways in which war is described. Students must understand the main   themes, the key words and their meaning; they must look for rhetorical   devices and try to interpret the message of the poems. \\ \hline
5d   & 2    & 1      & Students should practice their knowledge of key events of the XXth   century they discussed in class. Specifically, they know the key following   facts about 3 main topics: 1- 1967 as Annus Mirabilis 1967 was an annus   mirabilis as regards sexual mores: Abortion Act National Health Service   (Family Planning) Act (local authorities provide contraceptives) Sexual   Offences Act(It decriminalised homosexual acts in private between two men   over 21) Divorce Act (1969) Matrimonial Property Act (1970) (the wife’s work   was regarded as an equal contribution towards creating the Family home) 2-   WW2 Participants: World War II (1939-45), major belligerents - Axis (Germany,   Italy, Japan) vs Allies (France, Britain, USA, Soviet Union, China). Initial   Events: 1938, Germany annexes Czechoslovakia; 1939, invades Poland,   triggering WWII. Turning Points: Failure of Germany to control air, 1940.   Invasion of USSR by Germany, 1941; severe losses due to Russian winter and   resistance. USA enters war, 1941 post-Pearl Harbor attack. Conclusion: D-Day,   1944: Allied forces land in Normandy. Germany surrenders, 1945, post-Hitler’s   suicide. USA drops atomic bombs on Hiroshima, Nagasaki, 1945, leading to   Japan's surrender. 3- Margaret Thatcher 4th May 1979: Margaret Thatcher   (right wing of theConservative Party) became Prime Minister. She tried to   solve the UK’s economic decline and to reduce the role of the state in the   economy.                                                   & Questions on the 20th century     & Students are asked to answer one open question for each of the following   topics: 1. 1967, annus mirabilis 2. Key points of WW2 3. Margaret Thatcher                                                                                                                                                                                                                                                                                        \\ \hline
5d   & 3    & 1      & Students should practice their knowledge of key events of the 20s in the   US they discussed in class. Specifically, they know the key following facts   about 4 main topics: 1- Economical changes Reasons for prosperity in the 20s:   Impact of the car industry Impact of Ford’s assembly line Development of car,   electrical and radio and motion picture industry,  Consequences: economical boom, Mass   consumption  2- political changes  US between 1920-1930 was led by Republican   presidents that try to return to normality after WWI Under president Hoover   there was the Wall Street Crash (Black Tuesday) in 1929 Beginning of the   Great Depression  3- social Changes   1919: 18th amendment and beginning of prohibition: bootlegging 1920: 19th   amendment: women can vote 1933 21st amendment made alcohol legal again   Speakeasies and flappers Nativism and racism     4-  F. S. Fitzgerald: The Great   Gatsby Main points of his life: Zelda, excess, the Lost Generation The Great   Gatsby: main characters  The Great   Gatsby: setting (Valley of Ashes, East/West Eggs, New York The Great Gatsby:   main themes (old money v new money,, self-made man, cars, the American dream)   The Great Gatsby: symbols (green light, Valley of Ashes, East/West Eggs)                                                                                                                                                                                                                                                           & Questions on the Roaring 20s      & Students are asked to answer one open question for each of the following   topics: 1. Reasons for prosperity in the US 20s 2. Great Depression 3.   Prohibition 4. The Great Gatsby                                                                                                                                                                                                                                                          \\ \hline
5d   & 4    & 1      & Students should practice their knowledge of key events after WWII  in the US they discussed in class.   Specifically, they know the key following facts about 4 main topics: Cold   War:  Dates countries involved Reasons   The Swinging Sixties: Some key dates: 1961: Kennedy’s election and the   Soviet’s first manned spaceflight 1962: Nuclear showdown with Cuba 1963:   Kennedy’s assassination 1964: Civil Rights Act 1969: USA moon landing The   cultural revolution: drugs, discos,    progressiveness in education, pop music and poetry, one-parent   families,  the contraceptive pill,   abortion homosexuality legalised. The decay of the 70s: 1959-75 Vietnam War   and protests 1972-1974: The Watergate scandal 1970s: Carter’s administration   was marked by stagflation (stagnation+inflation = slow economic growth and   rising prices) ‘Me’ decade    Individualism, selfishness, punk culture, political struggle,   radicalism (no pacifism), racism, nihilism                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & Open Questions                    & Students are asked to answer one open question for each of the following   topics: 1. Main reasons and beginning of cold War 2. Most important dates of   the 60s in the US with main events 3. Essential aspects of the US cultural   revolution 4. Crisis of the 70s                                                                                                                                                                       \\ \hline
5d   & 5    & 1      & Students should practice their knowledge of the most important activists   for Human Rights they discussed in class. Specifically, they know the key   following facts about the following main topics:  Gandhi’s life: In May 1883, he was married   to 14-year old girl (arranged marriage) In 1888 Gandhi travelled to London,   to study law at University College London and to train as a lawyer. His   attempts at establishing a law practice in Mumbai failed. In 1893 he went to   South Africa and faced discrimination (concept of apartheid) In 1920 he   became leader of the Indian National Congress In 1934 he resigned not only as   the leader but also as a member of theCongress Party. Gandhi was assassinated   in 1948 2. Gandhi’s main achievements and influence The non violent   resistance: satyagraha. His methods included writing speeches and letters   leading marches organizing protests and demonstrations boycotting British   goods and institutions leading prayer meetings 1930: the Salt March: a   satyagraha against the British-imposed tax on salt, which affected the   poorest section of the community. It resulted in the imprisonment of more   than 60,000 people. Quit India: This was Gandhi's and the Congress Party's   most definitive revolt aimed at securing the British exit from India.   formation of the two new dominions of India and Pakistan in mid-August 1947.   His Legacy of nonviolence and civil rights influenced many leaders worldwide   such as Nelson Mandela and M.L. King Jr. & Open Questions                    & Students are asked to answer 5 open questions on Gandhi’s life and   achievements.                                                                                                                                                                                                                                                                                                                                                           \\ \hline
5d   & 6    & 1      & Students should practice their knowledge of the most important women in   history they discussed in class. Specifically, they know the key following   facts about the following main topics: Queen Victoria:  Values Reforms apex of the British   empire  Emmeline Pankhurst and women’s   right to vote:  1903: Women’s Social   and Political Union 1918: Representation of the People Act  1928: Equal Franchise Act 1928   Suffragettes: definition of the concepts 1920: The Nineteenth Amendment Rosa   Parks: Rebellion against governmental laws in 1955 Bus boycott repercussions                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & Open Questions\label{tab:exercises}                    & Students are asked to answer one open question for each of the following   topics: 1. Queen Victoria 2. Emmeline Pankhurst 3. Rosa Parks                                                                                                                                                                                                                                                                                                     \\ \hline



\end{longtable}
\end{scriptsize}

==> tables/factors.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Factor & 1st & 2nd & 3rd & 4th & 5th \\
\hline
Factor 1 & ability_keep_up_sum (-0.855) & confidence_in_ability_sum (-0.848) & cant_learn_english_sum (0.836) & doubt_difficult_topics_sum (0.836) & confident_in_tests_sum (-0.812)  \\
\hline
Factor 2 & lessons_improved_english_sum (-0.79) & homework_future_knowledge_sum (-0.735) & overall_satisfaction_sum (-0.728) & homework_improves_english_sum (-0.709) & lessons_future_knowledge_sum (-0.685)  \\
\hline
Factor 3 & uninterested_in_content_sum (-0.48) & need_support_homework_sum (-0.413) & homework_boring_sum (-0.405) & confidence_in_ability_sum (-0.371) & good_at_languages_sum (-0.327)  \\
\hline
Factor 4 & goal_c1_english_sum (-0.566) & struggled_with_english_sum (-0.315) & confident_in_tests_sum (0.265) & ability_keep_up_sum (0.261) & ability_finish_homework_sum (0.257)  \\
\hline
Factor 5 & skip_hard_topics_sum (0.587) & skip_hard_exercises_sum (0.413) & overall_satisfaction_sum (0.25) & goal_c1_english_sum (-0.249) & homework_improves_english_sum (-0.209)  \\
\hline
\end{tabular}

==> tables/weekly.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{|c|c|cc|cc|c|}
\hline
\rowcolor[HTML]{333333} 
\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} }                                                                       & \cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} }                                                                    & \multicolumn{2}{c|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \TU}}                               & \multicolumn{2}{c|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \TI}}                                 & \cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} }                                    \\ \cline{3-6}
\rowcolor[HTML]{333333} 
\multirow{-2}{*}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}From \\ Week\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \begin{tabular}[c]{@{}c@{}}To\\ Week\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} Cohen's d}} & {\color[HTML]{FFFFFF} P-value} & \multicolumn{1}{c|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} Cohen's d}} & {\color[HTML]{FFFFFF} P-value} & \multirow{-2}{*}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} Number of Samples}} \\ \hline
1                                                                                                                     & 2                                                                                                                  & \multicolumn{1}{c|}{0.039}                                                  & 0.833                          & \multicolumn{1}{c|}{0.128}                                                    & 0.575                          & 24                                                                                 \\
1                                                                                                                     & 3                                                                                                                  & \multicolumn{1}{c|}{-0.371}                                                 & 0.083                          & \multicolumn{1}{c|}{-0.045}                                                   & 0.877                          & 22                                                                                 \\
1                                                                                                                     & 4                                                                                                                  & \multicolumn{1}{c|}{-0.242}                                                 & 0.172                          & \multicolumn{1}{c|}{-0.167}                                                   & 0.547                          & 18                                                                                 \\
1                                                                                                                     & 5                                                                                                                  & \multicolumn{1}{c|}{-0.068}                                                 & 0.806                          & \multicolumn{1}{c|}{0.000}                                                    & 1.000                          & 16                                                                                 \\
1                                                                                                                     & 6                                                                                                                  & \multicolumn{1}{c|}{-0.539}                                                 & 0.086                          & \multicolumn{1}{c|}{0.057}                                                    & 0.858                          & 19                                                                                 \\
2                                                                                                                     & 3                                                                                                                  & \multicolumn{1}{c|}{-0.373}                                                 & 0.163                          & \multicolumn{1}{c|}{-0.219}                                                   & 0.449                          & 18                                                                                 \\
2                                                                                                                     & 4                                                                                                                  & \multicolumn{1}{c|}{-0.191}                                                 & 0.509                          & \multicolumn{1}{c|}{-0.288}                                                   & 0.352                          & 16                                                                                 \\
2                                                                                                                     & 5                                                                                                                  & \multicolumn{1}{c|}{-0.366}                                                 & 0.219                          & \multicolumn{1}{c|}{0.137}                                                    & 0.584                          & 13                                                                                 \\
2                                                                                                                     & 6                                                                                                                  & \multicolumn{1}{c|}{-0.371}                                                 & 0.138                          & \multicolumn{1}{c|}{-0.244}                                                   & 0.450                          & 17                                                                                 \\
3                                                                                                                     & 4                                                                                                                  & \multicolumn{1}{c|}{0.115}                                                  & 0.579                          & \multicolumn{1}{c|}{-0.113}                                                   & 0.651                          & 17                                                                                 \\
3                                                                                                                     & 5                                                                                                                  & \multicolumn{1}{c|}{-0.077}                                                 & 0.779                          & \multicolumn{1}{c|}{0.078}                                                    & 0.796                          & 11                                                                                 \\
3                                                                                                                     & 6                                                                                                                  & \multicolumn{1}{c|}{-0.229}                                                 & 0.427                          & \multicolumn{1}{c|}{-0.497}                                                   & 0.131                          & 13                                                                                 \\
4                                                                                                                     & 5                                                                                                                  & \multicolumn{1}{c|}{-0.519}                                                 & 0.030*                          & \multicolumn{1}{c|}{0.463}                                                    & 0.140                          & 7                                                                                  \\
4                                                                                                                     & 6                                                                                                                  & \multicolumn{1}{c|}{-0.598}                                                 & 0.152                          & \multicolumn{1}{c|}{-0.210}                                                   & 0.623                          & 12                                                                                 \\
5                                                                                                                     & 6                                                                                                                  & \multicolumn{1}{c|}{-0.198}                                                 & 0.586                          & \multicolumn{1}{c|}{-0.077}                                                   & 0.838                          & 12                                                                                 \\ \hline
\end{tabular}
\caption{Paired t-tests for self reported \TI and \TU across weeks}
\label{tab:int}
\end{table}

